Quality at the Tail of Machine Learning Inference

Machine learning inference should be subject to stringent inference time constraints while ensuring high inference quality, especially in safety-critical (e.g., autonomous driving) and mission-critical (e.g., emotion recognition) contexts. Neglecting either aspect can lead to severe consequences, such as loss of life and property damage. Many studies lack a comprehensive consideration of these metrics, leading to incomplete or misleading evaluations. The study unveils a counterintuitive revelation: deep learning inference quality exhibits fluctuations due to inference time. To depict this phenomenon, the authors coin a new term, "tail quality," providing a more comprehensive evaluation, and overcoming conventional metric limitations. Moreover, the research proposes an initial evaluation framework to analyze factors affecting quality fluctuations, facilitating the prediction of the potential distribution of inference quality. The effectiveness of the evaluation framework is validated through experiments conducted on deep learning models for three different tasks across four systems.

==> sections/motivation.tex <==
% !TEX root = ../main.tex
\section{Motivation}
\subsection{Why the metric of tail quality is essential?}
Relying solely on inference quality or tail latency as metrics to assess the inference capability of deep learning is insufficient.
Specifically, as depicted in Figure~\ref{fig:tail_quality}, an experiment is conducted using an image classification model ViT on a Tesla P100.

When there are no constraints on inference time, the deep learning model's inference quality is 81.512\%, with a 99th percentile tail latency of 472.41 ms.
These two metrics are commonly employed in deep learning research: accuracy serves as an evaluation metric for model inference quality, while tail latency is used to gauge the stability of deep learning systems.

However, when tail quality is adopted as an evaluation metric and the inference time threshold is set to the 99th percentile tail latency (i.e., 99\% tail quality @ 472.41 ms), the tail quality decreases from its original value of 81.512\% to 79.80\%, with fluctuations ranging between 79.80\% and 81.14\%.
Moreover, setting the threshold at the 90th percentile tail latency leads to more pronounced fluctuations in tail quality (i.e., 90\% tail quality @ 392 ms fluctuates from 68.26\% to 76.78\%).

These variations in inference quality due to inference time cannot be adequately captured solely by using traditional inference quality and tail latency metrics.
Hence, utilizing tail quality as an evaluation metric is of paramount importance.
% ``Tail quality'' refers to the inference quality situated at the tail of a distribution when fluctuations occur in inference quality.
% It characterizes the quality of inference results under the constraint of inference time, depicting the extent of the goodness of inference results when inference time limitations influence the inference process.
% Many tasks impose stringent constraints on inference time in the real world.
% If the processing duration of the inference process exceeds the designated inference time, it can lead to highly severe consequences.
% % In the practical application of deep learning, nearly all scenarios demand a certain level of inference speed from the deep learning models.
% This urgency is particularly pronounced in critical tasks.
% Take high-frequency trading as an example, where buying and selling activities occur within extremely short time intervals, often measured in milliseconds or even microseconds.
% High-frequency trading operates in an environment of rapid market fluctuations, where information like prices and orders can quickly change.
% As a result, delayed decisions could potentially result in significant financial losses.

% As mentioned in the introduction, autonomous driving is also a prime example.
% When numerous deep learning models are applied in autonomous driving, ensuring their exceptional stability is essential to prevent misjudgments and inefficient inferences.
% This is because, as a safety-critical task, deep learning model inference has strict requirements for response time.
% Even if the inference results are correct, an inference is unsuccessful if the inference time surpasses the threshold.
% If the inference time exceeds the specified threshold by just tens of milliseconds, a vehicle traveling within a speed range of 60 km/h to 180 km/h would have already moved half a meter or several meters during the exceeded time.

% Additionally, quality evaluation metrics for deep learning are based on assessing the model's inference results on specific test datasets.
% However, in practical applications, due to the constraint of inference time, even if the model performs well on the test dataset, if the entire deep learning inference process cannot consistently operate within a limited time frame, the occurrence of a single failure among ten thousand inferences suggests an issue with the deep learning inference capability.
% The quality fluctuations induced by limited inference time must be treated with the highest concern to avert the severe consequences in real-world applications.
% Hence, research on ``tail quality'' carries substantial significance.

% % \subsection{Difference between Tail Quality and Other Metrics}


 \subsection{Why need a tail quality evaluation framework?}
In critical tasks, the fluctuation in tail quality of deep learning inference at a specific threshold can significantly impact its practical applications.
Lower tail quality values might lead to irreversible and severe consequences.
For instance, in domains like autonomous driving or high-frequency trading systems, the constraints on inference time can be extremely stringent.
In the event of inference failure, the consequences could involve loss of life and property.
Hence, there's a need to predict the phenomenon of tail quality and analyze its underlying causes.

However, constructing methods for prediction and analysis presents numerous challenges.

Modeling aspects such as inference quality, inference time, and the various components of deep learning proves to be highly difficult.
Based on the premise, and with the revelation of \emph{``tail quality''} and its implication of the dependency between inference quality and inference time, benchmarking and evaluation of deep learning inference have become even more complex.

Therefore, the construction of accurate tail quality prediction and analysis models while keeping computational resource costs low is of paramount importance, yet it remains a challenging endeavor.

==> tables/sys_specs.tex <==
\begin{table*}[tb]
\centering
\caption{Detailed System Configurations}
\label{tab:sys_specs}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{cc||cccc}
\hline
\multicolumn{2}{c||}{\textbf{Specs}}           & \multicolumn{1}{c|}{\textbf{Server A}} & \multicolumn{1}{c|}{\textbf{Server B}} & \multicolumn{1}{c|}{\textbf{Server C}} & {\textbf{Server D}} \\ \hline\hline
\multicolumn{1}{c|}{\multirow{5}{*}{GPU}} & Type & \multicolumn{1}{c|}{GeForce RTX 2080 Ti} & \multicolumn{1}{c|}{TITAN V} & \multicolumn{1}{c|}{Tesla P100} & Tesla V100 \\ \cline{2-6} 
\multicolumn{1}{c|}{} & Cores        & \multicolumn{1}{c|}{4352}     & \multicolumn{1}{c|}{5152}     & \multicolumn{1}{c|}{3584}     & 5120     \\ \cline{2-6} 
\multicolumn{1}{c|}{} & Memory       & \multicolumn{1}{c|}{11GB}     & \multicolumn{1}{c|}{12GB}     & \multicolumn{1}{c|}{16GB}     & 32GB     \\ \cline{2-6} 
\multicolumn{1}{c|}{} & Amount       & \multicolumn{1}{c|}{4}        & \multicolumn{1}{c|}{1}        & \multicolumn{1}{c|}{1}        & 1        \\ \cline{2-6} 
\multicolumn{1}{c|}{} & Architecture & \multicolumn{1}{c|}{Turing}   & \multicolumn{1}{c|}{Volta}    & \multicolumn{1}{c|}{Pascal}   & Volta    \\ \cline{2-6} 
\multicolumn{1}{c|}{} & CUDA Version & \multicolumn{1}{c|}{11.7}   & \multicolumn{1}{c|}{11.7}    & \multicolumn{1}{c|}{11.6}   & 11.7    \\ \hline
\multicolumn{2}{c||}{PyTorch}             & \multicolumn{4}{c}{1.12.1}                                            \\ \hline
\multicolumn{2}{c||}{TensorFlow}             & \multicolumn{4}{c}{2.13.0}                                            \\ \hline
\multicolumn{2}{c||}{CPU}             & \multicolumn{4}{c}{Intel(R) Xeon(R) CPU E5-2620 v3 @   2.40G}                                            \\ \hline
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}%
